Resource Allocation in HyperX Networks

As high-performance computing systems scale in size and complexity, efficient resource management is essential to minimize communication overhead. The HyperX is a richly connected, low-diameter network that offers a scalable and cost-effective alternative to traditional topologies. However, resource allocation in HyperX remains underexplored, and strategies designed for networks like Torus, Fat-tree, or Dragonfly do not directly transfer. In this work, we propose and formalize several resource allocation strategies for HyperX networks, categorized into linear, geometric, and stochastic functions. We characterize these strategies theoretically by analyzing their topological properties, including dilation, convexity, and partition bandwidth.Furthermore, we conduct an exhaustive experimental evaluation using synthetic traffic and application communication kernels to assess the impact of these strategies on performance under different routing algorithms. Our results indicate that partition bandwidth and switch locality are decisive factors in mitigating interferences. Notably, the Diagonal allocation strategy, which is not convex, consistently outperforms traditional approaches in most scenarios. Finally, we provide a set of lessons learned to guide the implementation of resource allocation policies in HPC systems based on HyperX networks.

==> figures/topologias.tex <==


\makeatletter
\newcommand{\dgflydraw}[7]{%
	\xdef\a{#1}%
	\xdef\b{#2}%
	\xdef\Dg{#3}%
	\xdef\t{#4}%
	\pgfmathparse{360/\b}
	\global\let\gangle=\pgfmathresult
	%
	%
	%
	%
	\pgfmathsetlengthmacro{\groupwidth}{1.3*#6/\b}%
	\pgfmathsetlengthmacro{\groupnodewidth}{\groupwidth}%
	%
	%
	\pgfmathsetlengthmacro{\seprouters}{1.55*\groupwidth/\a}%
	\pgfmathsetlengthmacro{\routernodewidth}{.9*\seprouters-1pt}%
	%
	%
	%
	%
	%
	%
	\pgfmathparse{int(\a-1)}
	\global\let\Pa=\pgfmathresult
	\pgfmathparse{int(\b-1)}
	\global\let\Pb=\pgfmathresult
	\pgfmathparse{int(\b-2)}
	\global\let\PPb=\pgfmathresult
	\pgfmathparse{int(\Dg-1)}
	\global\let\Pdg=\pgfmathresult
	\pgfmathparse{int(\t-1)}
	\global\let\Pt=\pgfmathresult
	\csname dgfly@configuration@#5\endcsname
	\begin{tikzpicture}[
		scale=1.2,
		switch/.style={
			draw=black!80, circle, thick, fill=white,
			inner sep=0pt, minimum width=5pt,
			font=\scriptsize\sffamily
		},
		server/.style={
			draw=gray!60, rectangle, rounded corners=1pt, fill=gray!20,
			inner sep=0pt, minimum width=4pt, minimum height=2.5pt
		},
        cable/.style={draw=black, line width=0.5pt},
        serverlink/.style={draw=black, line width=0.3pt},
		group/.style={inner sep=0pt,rectangle,minimum width=\groupnodewidth,minimum height=.5*\groupnodewidth},
		%
		%
		%
		link/.style={cable}
		]%
	%
	\foreach \ig in {0,...,\Pb} {
		\path ++(-90+\ig*\gangle:.35*#6) node[group,rotate=\ig*\gangle](group\ig)  {};
		\begin{scope}[transform shape,rotate=\gangle*\ig]
		\foreach \ia in {0,...,\Pa} {
			\path (group\ig) ++(0:{0.5*\seprouters-0.5*\a*\seprouters}) ++(\ia*\seprouters,0) node[switch](router\ig_\ia) {};
			\expandafter\xdef\csname style\ig_\ia\endcsname{}
                        \foreach \is in {-1,1} {
                           \node[server,xshift=\is*2pt,below=3pt of router\ig_\ia] (server\ig_\ia_\is) {};
                           \draw[link] (router\ig_\ia) -- (server\ig_\ia_\is);
                        }
		}
                \draw (router\ig_0) -- (router\ig_1) (router\ig_1) -- (router\ig_2) (router\ig_2) -- (router\ig_3);
                \draw (router\ig_0) .. controls +(0.1,0.35) and +(-0.1,0.35) ..  (router\ig_2)
                      (router\ig_1) .. controls +(0.1,0.35) and +(-0.1,0.35) ..  (router\ig_3);
                \draw (router\ig_0) .. controls +(0,0.5) and +(0,0.5) ..  (router\ig_3);
		\end{scope}
	}
	\node[anchor=north] at (server0_1_1.south) {#7};
	\foreach \ia in {0,...,\Pa}
	\foreach \ih in {0,...,\Pdg}
	{
		%
		%
	}
	\foreach \ig in {0,...,\Pb}
	{
		\foreach \ia in {0,...,\Pa}
		{
			\foreach \ih in {0,...,\Pdg}
			{
				%
				%
				\dgflylink{\ig}{\ia}{\ih}
				%
				%
				%
				%
				%
				%
				%
				%
				\ifthenelse{\resultb>\ig}
				{
					\draw[link,
						\csname style\ig_\ia\endcsname,
						\csname style\resultb_\resulta\endcsname,
						] (router\ig_\ia) -- (router\resultb_\resulta);
				}{}
			}
		}
	}
	%
	\end{tikzpicture}
}
\newcommand{\palmtree@link}[3]{%
	\edef\ig{#1}
	\edef\ia{#2}
	\edef\ih{#3}
	\pgfmathparse{int(\a-\ia-1)}
	\xdef\resulta{\pgfmathresult}
	\pgfmathparse{int(mod(\ig+1+mod(\resulta*\Dg+\ih,\b-1),\b))}
	\xdef\resultb{\pgfmathresult}
}
\newcommand\dgfly@configuration@palmtree{%
	\global\let\dgflylink=\palmtree@link
}
\makeatother





\begin{figure*}[tb]
	\centering%
	\begin{tikzpicture}[
		switch/.style={
			draw=black!80, circle, thick, fill=white,
			inner sep=0pt, minimum width=5pt,
			font=\scriptsize\sffamily
		},
		server/.style={
			draw=gray!60, rectangle, rounded corners=1pt, fill=gray!20,
			inner sep=0pt, minimum width=4pt, minimum height=2.5pt
		},
        cable/.style={draw=black, line width=0.5pt},
        serverlink/.style={draw=black, line width=0.3pt},
	]
	\begin{scope}[
		x=0.3cm, y=1.7cm,
		yshift=1cm,
	]
		\def\k{3} %
		\def\l{3} %
		\pgfmathtruncatemacro\kP{\k-1}
		\pgfmathtruncatemacro\lP{\l-1}
		\pgfmathtruncatemacro\lPP{\l-2}
		\pgfmathtruncatemacro\lPPP{\l-3}
		\pgfmathtruncatemacro\n{\k^(\l-1)} %
		\pgfmathtruncatemacro\nP{\n-1}
		\pgfmathtruncatemacro\nn{\n+\n}
		\pgfmathtruncatemacro\nnP{\nn-1}
		\foreach \x in {0,...,\nnP}
		{
		\foreach \y in {0,...,\lPP}
		{
			\node[switch](switch \x_\y) at (\x,\y*0.7) {};
		}
		}
		%
		\foreach \x in {0,...,\nP}
		{
			%
			\node[switch](switch \x_\lP) at (2*\x+0.5,\lP+0.0) {};
		}
		\foreach \x in {0,...,\nnP}
		\foreach \ik in {0,...,\kP}
		{
			\pgfmathsetmacro\tmp{\x+(\ik+.5)/\k-.5}
			%
			\node[server] (server \x_\ik) at (\tmp,-10pt) {};
			\draw[serverlink] (server \x_\ik) -- (switch \x_0);
		}
		\foreach \y in {0,...,\lPPP}
		{
			\pgfmathtruncatemacro\s{\k^\y}
			\pgfmathtruncatemacro\g{\s*\k}
			\pgfmathtruncatemacro\yN{\y+1}
			\foreach \a in {0,...,\nnP}
			\foreach \ik in {0,...,\kP}
			{
				\pgfmathtruncatemacro\b{ mod(\a+\s*\ik,\g) + int(\a/\g)*\g }
				%
					\draw[cable] (switch \a_\y) -- (switch \b_\yN);
			}
		}
		%
		\pgfmathtruncatemacro\s{\k^\lPP}
		\pgfmathtruncatemacro\g{\s*\k}
		\foreach \a in {0,...,\nnP}
		\foreach \ik in {0,...,\kP}
		{
			\pgfmathtruncatemacro\b{ mod( mod(\a+\s*\ik,\g) + int(\a/\g)*\g  , \n )}
			%
			\draw[cable] (switch \a_\lPP) -- (switch \b_\lP);
		}
	\end{scope}
	\begin{scope}[xshift=7cm,yshift=.5cm,scale=1.2,
		%
		x={(0.7cm,0.2cm)},
		y={(0.0cm,0.6cm)},
		z={(-0.3cm,0.3cm)},
		xhighlight/.style={green!50!black,solid,very thick},
		yhighlight/.style={blue,solid,very thick},
		zhighlight/.style={red!50!black,solid,very thick},
		]
		%
		\foreach \j in {3,...,0}
		\foreach \i in {0,...,3}
		\foreach \k in {0,...,3}
		{
		\path (\i,\k,\j) node[switch] (nodo_\i_\j_\k) {};
		}
		\begin{scope}[overlay,very thin,
		normal/.style={cable},
		]
		\foreach \j in {3,...,0}
		\foreach \i in {0,...,3}
		\foreach \k in {0,...,3}
		{
		\pgfmathtruncatemacro\nexti{mod(\i+1,4)}
		%
		%
		%
		%
		%
		%
		\ifthenelse{\i=3}{
			\draw[densely dotted,normal] (nodo_\i_\j_\k) edge[out=20-15,in=190+15] (nodo_\nexti_\j_\k);
		}{
			\draw[normal] (nodo_\i_\j_\k) -- (nodo_\nexti_\j_\k);
		}
		\pgfmathtruncatemacro\nextj{mod(\j+1,4)}
		%
		%
		%
		%
		%
		%
		\ifthenelse{\j=3}{
			\draw[densely dotted,normal] (nodo_\i_\j_\k) edge[out=140,in=-60] (nodo_\i_\nextj_\k);
		}{
			\draw[normal] (nodo_\i_\j_\k) -- (nodo_\i_\nextj_\k);
		}
		\pgfmathtruncatemacro\nextk{mod(\k+1,4)}
		%
		%
		%
		%
		%
		%
		\ifthenelse{\k=3}{
			\draw[densely dotted,normal] (nodo_\i_\j_\k) edge[out=80,in=-80] (nodo_\i_\j_\nextk);
		}{
			\draw[normal] (nodo_\i_\j_\k) -- (nodo_\i_\j_\nextk);
		}
		}
		\end{scope}
	\end{scope}
	%
	%
	%
	%
	\end{tikzpicture}%
	\hspace{1cm}%
	\dgflydraw{4}{9}{2}{1}{palmtree}{24ex}{}
	\caption{%
		%
		Three topologies employed in HPC. From left to right: a 54-server, 6-radix, 3-level Fat-tree, a $4\times 4\times 4$ torus, and a Dragonfly with 9 groups.
		Endpoints in Torus are omitted, but each switch is supposed to be connected to one endpoint.
		}
	\label{fig:topologias}
\end{figure*}


